Unveiling and Harnessing Hidden Attention Sinks: Enhancing Large Language Models without Training through Attention Calibration

Attention is a fundamental component behind the remarkable achievements of large language models (LLMs). However, our current understanding of the attention mechanism, especially regarding how attention distributions are established, remains limited. Inspired by recent studies that explore the presence of attention sink in the initial token, which receives disproportionately large attention scores despite their lack of semantic importance, this work delves deeper into this phenomenon. We aim to provide a more profound understanding of the existence of attention sinks within LLMs and to uncover ways to enhance the achievable accuracy of LLMs by directly optimizing the attention distributions, without the need for weight finetuning. Specifically, this work begins with comprehensive visualizations of the attention distributions in LLMs during inference across various inputs and tasks. Based on these visualizations, to the best of our knowledge, we are the first to discover that (1) attention sinks occur not only at the start of sequences but also within later tokens of the input, and (2) not all attention sinks have a positive impact on the achievable accuracy of LLMs. Building upon our findings, we propose a training-free Attention Calibration Technique (ACT) that automatically optimizes the attention distributions on the fly during inference in an input-adaptive manner. Extensive experiments validate that ACT consistently enhances the accuracy of various LLMs across different applications. Specifically, ACT achieves an average improvement of up to 7.30% in accuracy across different datasets when applied to Llama-30B. Our code is available at https://github.com/GATECH-EIC/ACT.

==> sections/1-introduction.tex <==
\section{Introduction}
% LLMs are powerful, but improving the performance of LLMs is a long-lasting topic 
In recent days, large language models (LLMs) have drawn significant attention because of their impressive performance in a wide range of tasks~\cite{} that comes with their gigantic model size, making LLMs the foundation of many applications that change people's lives. The increasing demand for powerful LLMs further motivates various attempts to improve the performance of LLMs on different tasks. 


% existing techniques need large resources for tuning (e.g., computation and mem) or inference (e.g., more iterations for inference)

However, due to the large model size of LLMs, improving the performance of LLMs at an affordable cost is a non-trivial challenge. Existing approaches for performance improvement either (1) fine-tune LLMs on downstream tasks or (2) optimize the generation process by constructing a better input. However, these methods suffer from the challenge of efficiency in different aspects, limiting the desired widespread application of LLMs. Specifically, (1) fine-tuning LLMs leads to exhaustive memory and computation overhead, even one of the state-of-the-art (SOTA) efficient tuning techniques still requires \zzyu{xxx GB of GPU memory and xxx GPU hours} to tune a medium-scale LLM (e.g., LLaMA-13B) on the SOTA A100 GPU, and (2) optimizing the generation usually leads to non-neglectable additional cost during inference. For example, SOTA prompting methods improve LLMs' performance on downstream tasks at the cost of \zzyu{$\sim$xxx times longer input prompt~\cite{}} while SOTA retrieval augmented generation techniques can lead to \zzyu{$\sim$33\% higher inference latency compared with the vanilla model~\cite{}}. 

% Recent works show attention can be a good identifier to improve LLM in specific tasks 
On the other hand, recent advances in LLM visualization~\cite{} and knowledge localization and editing of LLMs~\cite{} observe that attention maps generated during the inference process of LLMs contain much information depicting the way how LLMs are generating the output based on the key information contained in the input and the knowledge they have learned during the pretraining process. Moreover, some pioneering works show the possibility of improving the performance of LLMs on specific tasks (e.g., handling long input context) by modification on attention maps during inference. However, these works~\cite{} failed to achieve a consistent performance boost across a diverse range of applications and needed to label important parts of inputs manually~\cite{}, thus limiting their usability. 

Motivated by these observations, we aim to further explore the attention map's behavior during LLMs inference and answer the following research question: Can we identify the suspicious attention pattern automatically during inference and, by fixing these patterns on-the-fly, boost the LLMs' performance across a diverse range of applications with almost no additional cost? 

Through our exploration to answer the research problem above, we make the following contributions: 
\begin{enumerate}
    \item We observe that existing LLMs tend to pay strong attention to some tokens in the input context and many of the tokens with high attention not only contain limited information but also do not help with improving the LLMs' performance. 
\end{enumerate}
% we aim to develop generalizable technique to improve LLM performance with neglectable additional cost during inference. 

% Contribution
